Decentralized FaaS over Multi-Clouds with Blockchain based Management for Supporting Emerging Applications

Function-as-a-Service (FaaS) offers a streamlined cloud computing paradigm, but existing centralized systems suffer from vendor lock-in and single points of failure. We propose DeFaaS, a decentralized FaaS system leveraging blockchain technology and decentralized API management. DeFaaS addresses these limitations by establishing a secure, transparent registry of functions on a blockchain and enabling applications to discover and invoke them. This approach fosters scalability, flexibility, enhanced security, and improved reliability. Furthermore, DeFaaS's architecture extends beyond decentralized FaaS, supporting other distributed computing scenarios like dApps, volunteer computing, and multi-cloud service meshes. DeFaaS represents a significant advancement in decentralized computing with the potential to unlock a multitude of novel applications and use cases.

==> sections/sec-future-work.tex <==
\section{Future Work}

In this paper, we have explored feasibility on designing a decentralized FaaS platform for Web3. The efforts only scratch the surface of the emerging research direction that integrates the traditional cloud based environments with the Web3 applications empowered by the blockchains. Future research directions include: in-depth experiment evaluation, integration and performance comparison of different designs of decentralized event/message delivery systems, optimization of Web3 storage, development of benchmarking suits, workload characterization, etc. 

==> sections/sec-service-mesh.tex <==

\section{Blockchain-based Multi-cloud Service Mesh}\label{sec-blockchain-service-mesh}

The concept of service mesh~\cite{li2019service} is an extension of micro service.
Withe service mesh, a group of micro services are connected to form a processing pipeline.
Existing design and implementation of service mesh adopts the idea of software-defined network (SDN) to separate common functions and service specific functions.
This separation greatly improves micro services from various perspectives, such as efficient management and flexible deployment.
However, existing service mesh architecture does not support multi-cloud 
This greatly limits the use and adoption of service mesh when an application relies on micro services that belong to multiple cloud service providers.
This is especially important for Dapps and Web3 applications because of their decentralization nature, i.e., even if a single cloud service provider can provide all necessary services, it is better to use multiple cloud service providers.

\sln{} provides all essential functions to support service mesh cross multiple cloud service providers.
From architecture perspective, the \sln{} management blockchain serves as the coordinator of multiple control planes.
These control planes are managed by different cloud service providers, and each of them manages its own service mesh.
When a request is sent to a service provider, but its corresponding control plane cannot resolve corresponding information, it can query the management blockchain. 
